Sunspot rotation. I. A consequence of flux emergence

Context. Solar eruptions and high flare activity often accompany the rapid rotation of sunspots. The study of sunspot rotation and the mechanisms driving this motion are therefore key to our understanding of how the solar atmosphere attains the conditions necessary for large energy release. Aims. We aim to demonstrate and investigate the rotation of sunspots in a 3D numerical experiment of the emergence of a magnetic flux tube as it rises through the solar interior and emerges into the atmosphere. Furthermore, we seek to show that the sub-photospheric twist stored in the interior is injected into the solar atmosphere by means of a definitive rotation of the sunspots. Methods. A numerical experiment is performed to solve the 3D resistive magnetohydrodynamic (MHD) equations using a Lagrangian-Remap code. We track the emergence of a toroidal flux tube as it rises through the solar interior and emerges into the atmosphere investigating various quantities related to both the magnetic field and plasma. Results. Through detailed analysis of the numerical experiment, we find clear evidence that the photospheric footprints or sunspots of the flux tube undergo a rotation. Significant vertical vortical motions are found to develop within the two polarity sources after the field emerges. These rotational motions are found to leave the interior portion of the field untwisted and twist up the atmospheric portion of the field. This is shown by our analysis of the relative magnetic helicity as a significant portion of the interior helicity is transported to the atmosphere. In addition, there is a substantial transport of magnetic energy to the atmosphere. Rotation angles are also calculated by tracing selected fieldlines; the fieldlines threading through the sunspot are found to rotate through angles of up to 353 degrees over the course of the experiment.

==> bmpsize-test.tex <==
%%
%% This is file `bmpsize-test.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% bmpsize.dtx  (with options: `test')
%% 
%% This is a generated file.
%% 
%% Project: bmpsize
%% Version: 2009/09/04 v1.6
%% 
%% Copyright (C) 2006-2009 by
%%    Heiko Oberdiek <heiko.oberdiek at googlemail.com>
%% 
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either
%% version 1.3c of this license or (at your option) any later
%% version. This version of this license is in
%%    http://www.latex-project.org/lppl/lppl-1-3c.txt
%% and the latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of
%% LaTeX version 2005/12/01 or later.
%% 
%% This work has the LPPL maintenance status "maintained".
%% 
%% This Current Maintainer of this work is Heiko Oberdiek.
%% 
%% This work consists of the main source file bmpsize.dtx
%% and the derived files
%%    bmpsize.sty, bmpsize.pdf, bmpsize.ins, bmpsize.drv,
%%    bmpsize-base.sty, bmpsize-test.tex, bmpsize-dvips.def,
%%    bmpsize-dvipdfm.def, bmpsize-dvipdfmx.def.
%% 
\expandafter\ifx\csname NeedsTeXFormat\endcsname\relax
  \input miniltx\relax
\fi
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname pdfoutput\endcsname\relax
\else
  \pdfoutput=0 %
\fi
\RequirePackage{bmpsize}

\endlinechar=-1
\catcode`\@=11
\def\msg#{\immediate\write16}

\def\init{%
  \msg{}%
  \msg{File name menu}%
  \msg{==============}%
  \msg{* Option menu: use `opt' as file name}%
  \msg{* Quit program: <return>}%
  \msg{}%
  \message{Image file name = }%
  \read-1 to \imagename
  \ifx\imagename\@empty
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {%
    \csname @@end\endcsname
    \end
  }{%
    \ifnum\pdf@strcmp{\imagename}{opt}=\z@
      \expandafter\optionmenu
    \else
      \startimg
      \expandafter\init
    \fi
  }%
}
\def\optionmenu{%
  \msg{}%
  \msg{Option menu}%
  \msg{===========}%
  \msg{Current setting:}%
  \msg{* bmpsizefast = \if@bmpsize@fast true\else false\fi}%
  \msg{* \if@bmpsize@user@resolution\else default\fi resolution = %
    \bmpsize@pixelx@default
    \space
    \bmpsize@pixely@default
  }%
  \msg{* \if@bmpsize@user@resolution default\fi resolution: not set}%
  \msg{* resolutionunit = \bmpsize@unit@default}%
  \msg{* Quit option menu: <return>}%
  \msg{}%
  \message{Options = }%
  \read-1 to \options
  \ifx\options\empty
    \expandafter\init
  \else
    \edef\@bmpsize@temp{%
      \noexpand\setkeys{Gin}{\options}%
    }%
    \@bmpsize@temp
    \expandafter\optionmenu
  \fi
}

\def\startimg{%
  \let\@found\@empty
  \msg{}%
  \msg{* File [\imagename]}%
  \@for\@type:=\bmpsize@types\do{%
    \ifx\@found\@empty
      \csname bmpsize@read@\@type\endcsname\imagename
      \ifbmpsize@ok
        \let\@found\@type
        \msg{\space\space Type: \@type}%
        \msg{\space\space Pixel width: \bmpsize@pixelwidth\space px}%
        \msg{\space\space Pixel height: \bmpsize@pixelheight\space px}%
        \ifx\bmpsize@pixelx\relax
        \else
          \ifx\bmpsize@unit\relax
            \let\@unit@spec\@empty
            \def\@ratio@name{Ratio }%
          \else
            \def\@unit@spec{\space dots per \bmpsize@unit}%
            \def\@ratio@name{Density }%
          \fi
          \msg{\space\space \@ratio@name x: \bmpsize@pixelx\@unit@spec}%
          \msg{\space\space \@ratio@name y: \bmpsize@pixely\@unit@spec}%
        \fi
        \msg{\space\space Width: \bmpsize@width\space bp}%
        \msg{\space\space Height: \bmpsize@height\space bp}%
        \ifx\bmpsize@orientation\relax
        \else
          \msg{\space\space Orientation: \bmpsize@orientation}%
        \fi
      \fi
    \fi
  }%
  \ifx\@found\@empty
    \edef\@file@date{\pdf@filemoddate{\imagename}}%
    \ifx\@file@date\@empty
      \msg{\space\space --> File not found <--}%
    \else
      \msg{\space\space --> Unknown image type <--}%
    \fi
  \fi
}

\ifx\noinit!\else\expandafter\init\fi
\endinput
%%
%% End of file `bmpsize-test.tex'.


==> hylatex.ltx <==
%
% hylatex.ltx
% Tanmoy Bhattacharya and Sebastian Rahtz, June 1995
%
% Use this file to make a format which includes the
% hyperref package in every LaTeX job.
%
% In web2c 7-based TeX world, we create the format file with
%   tex  -ini \&latex hylatex.ltx
% and then use with
%   tex \&hylatex
%
% In teTeX (TeX version 3.14159 (C version 6.1), LaTeX2e <1996/12/01>
% patch level 1), I create the format file with
%   initex \&latex hylatex.ltx
% and then use with
%   virtex \&hylatex
%
% This method is not supported by the LaTeX2e team, so
% I will try to find a better way. \AtBeginDocument does not
% work for reasons which I do not understand.
%
\makeatletter
\expandafter\everyjob\expandafter{\the\everyjob
 \typeout{ ********* Hyperref Macros loaded ******* }}
%
\expandafter\let\csname REAL document\endcsname\document
%
\def\document{%
 \endgroup
%
% NOTE:
% This setup sets up no options by default;
% change to suit your needs, by writing a hyperref.cfg control
% file.
%
 \RequirePackage{hyperref}
 \begingroup
 \@endpefalse\csname REAL document\endcsname
}
\makeatother
\dump


